Deep Transfer $Q$-Learning for Offline Non-Stationary Reinforcement Learning

In dynamic decision-making scenarios across business and healthcare, leveraging sample trajectories from diverse populations can significantly enhance reinforcement learning (RL) performance for specific target populations, especially when sample sizes are limited. While existing transfer learning methods primarily focus on linear regression settings, they lack direct applicability to reinforcement learning algorithms. This paper pioneers the study of transfer learning for dynamic decision scenarios modeled by non-stationary finite-horizon Markov decision processes, utilizing neural networks as powerful function approximators and backward inductive learning. We demonstrate that naive sample pooling strategies, effective in regression settings, fail in Markov decision processes.To address this challenge, we introduce a novel ``re-weighted targeting procedure'' to construct ``transferable RL samples'' and propose ``transfer deep $Q^*$-learning'', enabling neural network approximation with theoretical guarantees. We assume that the reward functions are transferable and deal with both situations in which the transition densities are transferable or nontransferable. Our analytical techniques for transfer learning in neural network approximation and transition density transfers have broader implications, extending to supervised transfer learning with neural networks and domain shift scenarios. Empirical experiments on both synthetic and real datasets corroborate the advantages of our method, showcasing its potential for improving decision-making through strategically constructing transferable RL samples in non-stationary reinforcement learning contexts.

==> 1-nota.tex <==



Let lowercase letter $x$, boldface letter $\bx$, boldface capital letter $\bX$, and blackboard-bold letter $\XX$ represent scalar, vector, matrix, and tensor, respectively. The calligraphy letter $\calX$ represents operator.
We use the notation $[N]$ to refer to the positive integer set $\braces{1, \ldots, N}$ for $N \in \ZZ_+$.
% We write by $a \asymp b$ when $a = \bigO{b}$ and $b = \bigO{a}$.
Let $C, c, C_0, c_0, \ldots$ denote generic constants, where the uppercase and lowercase letters represent large and small constants, respectively. The actual values of these generic constants may vary from time to time.
%As a convention, in this paper, we use upper case letters, such as $I$, $R$, and $M$, as the sizes of dimensions (fixed or growing). 
%We the corresponding lower case letters, e.g. $i$ and $m$, as the running indices which typically range from $1$ to their capital versions, e.g. $i \in [I]$ and $m\in [M]$
For any matrix $\bX$,  we use $\bx_{i \cdot}$, $\bx_{j}$, and $x_{ij}$ to refer to its $i$-th row, $j$-th column, and $ij$-th entry, respectively. 
All vectors are column vectors and row vectors are written as $\bx^\top$ for any vector $\bx$. 
For any two scalers $p$, $q$, we denote $p\wedge q := \min\{p,q\}$ and $p\vee q := \max\{p,q\}$.
% Notation $\bbone$ represents a vector or a matrix of all ones of proper size. 
% The set of $N\times K$ orthonormal matrices is defined as $\OO^{N \times K}$

Let $\nu_i$ be the $i$-th largest square root of eigenvalues of $\bX^\top \bX$, which are called the singular values of $\bX$. $\nu_{\max}$ (resp. $\nu_{\min}$) is the largest (resp. smallest) in absolute value among $\nu_i$. 
Use $\vect(\bX)$ as the vectorization of $\bX$, and define its inverse operator $\vect^{-1}(\bx)$ by $\vect^{-1}(\vect(\bX)) = \bX$. For two matrices $\bX_1\in\RR^{m\times n}$ and $\bX_2\in\RR^{p\times q}$, $\bX_1\otimes\bX_2\in\RR^{pm\,\times\,qn}$ is the Kronecker product. Note that $\vect(\bA\bX\bB)=(\bB^\top\otimes\bA)\vect(\bX)$. 
Denote $\diag(\bX_1,\bX_2)\in\RR^{(m+p)\times(n+q)}$ as the block-diagonal matrix with $\bX_1$ and $\bX_2$ being its diagonal blocks.

For any vector $\bx=(x_1,\ldots,x_p)^\top$, let $\|\bx\|:= \|\bx\|_2=(\sum_{i=1}^p x_i^2)^{1/2}$ be the $\ell_2$-norm, and let $\|\bx\|_1=\sum_{i=1}^p |x_i|$ be the $\ell_1$-norm. 
Besides, we use the following matrix norms: 
%maximum norm $\norm{\bX}_{max} := \underset{ij}{\max} \; \lvert x_{ij} \rvert$, $\ell_1$-norm $\norm{\bX}_1 := \underset{j}{\max} \sum_{i} \lvert x_{ij} \rvert$, $\ell_{\infty}$-norm $\norm{\bX}_{\infty} := \underset{i}{\max} \; \sum_{j} \lvert x_{ij} \rvert$, 
$\ell_2$-norm $\norm{\bX}_2 := \nu_{max}(\bX)$; $(2,1)$-norm $\norm{\bX}_{2,1} := \underset{\norm{\ba}_1=1}{\max} \norm{\bX\ba}_2 =\max_i \norm{\bx_{i}}_2$;
Frobenius norm $\|\bX\|_F = (\sum_{i,j}x_{ij}^2)^{1/2}$;
nuclear norm $\|\bX\|_*=\sum_{i=1}^n {\nu_{i}(\bX)}$.
When $\bX$ is a square matrix, we denote by $\Tr \paren{\bX}$, $\lambda_{max} \paren{\bX}$, and $\lambda_{min} \paren{\bX}$ the trace, maximum and minimum singular value of $\bX$, respectively.
For two matrices of the same dimension, define the inner product $\angles{\bX_1,\bX_2} = \Tr(\bX_1^\top \bX_2)$.
%In addition,  for matrix $\bX\in \RR^{p\times q}$, let $\bX^+\in\RR^{q\times p}$ be its  pseudo inverse.
%%define projection matrices $\bP_X^\perp = \bI - \bP_X$ and $\bP_X = \bX \paren{\bX^\top\bX}^{-1} \bX^\top$; 
%when $\bX^\top\bX$ is not inversible, then $\paren{\bX^\top\bX}^{+}$ means the Moore-Penrose generalized inverse of $\bX^\top\bX$.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
